Beyond Isolation: Unlocking Reinforcement Learning Component Synergy for Sample-Efficient Continuous Control

Reinforcement learning systems are significantly more complex than other machine learning paradigms due to inherent properties, causing RL system design to jointly account for many tightly coupled factors. Despite advances in individual algorithmic components, their functional interdependencies remain underexplored: do they exhibit mutual synergy or counterproductive interference? To bridge this gap, we conduct a systematic investigation and find that the efficacy of different components exhibits significant task-dependency, and naively stacking state-of-the-art techniques does not necessarily yield performance gains; instead, it often triggers emergent challenges, such as compounded non-stationarity. Building upon these findings, we distill a suite of actionable insights into the principled coordination of these components. Guided by these insights, we propose ROSER, an RL framework that coordinates three critical dimensions: Model-based Representation, Optimization Stability, and Experience Replay. Across diverse continuous-control benchmarks, ROSER consistently outperforms vanilla baselines and achieves 17.60% gains over naive stack. Our findings underscore the necessity of a holistic perspective in RL system design and paves the way for developing sample-efficient agents.

==> Section/7_RelatedWorks.tex <==
\section{Related Works}
\label{sec_relatedworks}

\paragraph{Representation Learning.}
% Learning effective representations is a long-standing topic in reinforcement learning and has been shown to play a crucial role in improving sample efficiency, particularly in environments with high-dimensional observations or partial observability.
% A wide range of methods introduce auxiliary objectives to shape representations, including contrastive learning, future prediction, and reward or dynamics modeling~\cite{jaderberg2017reinforcement,yarats2021contrastive,hafner2020dreamer}.

% Recent work has sought to better systematize this design space.
% In particular, \citet{nibridging} provide a unifying perspective on representation learning in RL by categorizing methods according to how representations encode state, history, and predictive information.
% They show that many successful approaches can be interpreted as self-predictive representation learning methods, where representations are optimized to predict future signals under different conditioning assumptions.
% This framework highlights that representation learning is not a monolithic technique, but rather a spectrum of design choices with distinct implications for stability, expressiveness, and downstream learning.

% In continuous-control settings, several methods have incorporated representation learning into actor-critic algorithms.
% TD-MPC~\cite{hansen2022tdmpc} and TD-MPC2~\cite{hansen2024tdmpc2} learn latent dynamics models to support planning-style updates, while MR.Q~\cite{fujimototowards} proposes to learn state and state--action embeddings via auxiliary prediction losses on rewards, dynamics, and termination signals.
% However, a recurring challenge across these approaches is the non-stationarity induced by evolving representations, particularly when learned embeddings are used as the sole inputs to policy and value networks.
% This non-stationarity can destabilize optimization and lead to highly task-dependent performance, motivating careful consideration of how learned representations are integrated with downstream components.


\paragraph{Optimization Stability.}
% Another line of work focuses on improving the stability and efficiency of optimization in deep reinforcement learning.
% Unlike supervised learning, RL optimization must contend with bootstrapped targets, non-stationary data distributions, and highly correlated updates, which often lead to unstable training dynamics.
% Prior studies have identified issues such as exploding feature norms, loss of plasticity, and sensitivity to reward scaling as major obstacles to stable learning~\cite{lyle2022plasticity,dohare2023loss}.

% To address these challenges, a variety of architectural and normalization techniques have been proposed.
% Residual connections, layer normalization, and carefully designed network parameterizations have been shown to improve gradient flow and stabilize learning~\cite{he2016resnet,ba2016layernorm}.
% Recent RL-specific architectures, such as SimBa~\cite{lee2025simba} and SimBaV2~\cite{lee2025hyperspherical}, further demonstrate that controlling feature norm growth and improving gradient conditioning can significantly enhance both stability and scalability in continuous control.
% These approaches highlight that architectural choices alone can have a profound impact on sample efficiency, even without modifying the underlying learning objective.

\paragraph{Experience Replay.}
Experience replay is a fundamental mechanism for improving data efficiency in off-policy reinforcement learning by reusing past interactions.
Uniform replay provides a simple and effective baseline, but has been shown to be suboptimal in many settings due to inefficient use of informative transitions.
Prioritized Experience Replay (PER)~\cite{schaul2015prioritized} addresses this limitation by sampling transitions based on temporal-difference error, while subsequent variants such as LAP~\cite{fujimoto2020equivalence} and LaBER~\cite{lahire2021large} further refine prioritization or batch construction to reduce variance and improve stability.
More recently, ReLo-based prioritization~\cite{sujit2022prioritizing} has been proposed as a principled alternative that prioritizes transitions according to their reducible loss, offering a closer approximation to the expected learning progress contributed by each sample.Empirical results suggest that such strategies can substantially improve sample efficiency across a range of tasks.

